Quest for precision in hadronic cross sections at low energy: Monte Carlo tools vs. experimental data

We present the achievements of the last years of the experimental and theoretical groups working on hadronic cross section measurements at the low energy e+e- colliders in Beijing, Frascati, Ithaca, Novosibirsk, Stanford and Tsukuba and on tau decays. We sketch the prospects in these fields for the years to come. We emphasise the status and the precision of the Monte Carlo generators used to analyse the hadronic cross section measurements obtained as well with energy scans as with radiative return, to determine luminosities and tau decays. The radiative corrections fully or approximately implemented in the various codes and the contribution of the vacuum polarisation are discussed.

==> abstract.tex <==
 We present last years achievements of the
experimental and theoretical groups working on hadronic cross section
 measurements and tau physics and 
    sketch the prospects in this
  fields for next few years to come. We describe the status
  of the Monte Carlo event generators used by the experimental
  collaborations
  at $e^+e^-$ machines with energies up to the energies of B-factories
  and for  analyses of tau decays,  and give an overview of the
  experimental results
  concerning hadronic cross section measurement and tau decays.
  We cover  experimental results and Monte Carlo generators concerning
  luminosity measurements, measurements of hadronic cross sections 
  using scan and radiative return method, and tau decays. 
   The accuracies of the Monte Carlo generators and their tests are
  overviewed. The available radiative corrections both included and not
  included in the codes are discussed. A special section is devoted to
  the vacuum polarisation contributions.  
  


